On-The-Fly Information Retrieval Augmentation for Language Models

Here we experiment with the use of information retrieval as an augmentation for pre-trained language models. The text corpus used in information retrieval can be viewed as form of episodic memory which grows over time. By augmenting GPT 2.0 with information retrieval we achieve a zero shot 15% relative reduction in perplexity on Gigaword corpus without any re-training. We also validate our IR augmentation on an event co-reference task.

==> exp_log.tex <==

\begin{comment}

\textbf{with all the previous Gigaword}:

zero-shot result (medium):

Without context: 34.3 \\
With context (full document): 26.1 \\

All remaining sentences with context (searched by sent 1): 29.5 \\
All remaining sentences with context (searched by sent 2): 28.0  \\

Whole document with context (searched by sent 1): 31.2 \\
Whole document with context (searched by sent 2): 29.4  \\

Without context-finetune: 23.03 \\

Whole document with context (searched by sent 1)-finetune: 23.01 \\
Whole document with context (searched by sent 2)-finetune:   \\


\ignore{

\textbf{PTB 3.0 dataset:} \\
\cite{ji2015document} also use the raw data as doc language model.
it doesn't have overlap with \cite{radford2019language} as demonstrated by GPT 2.0.

\textbf{Sent level}: \\
state of the art: 46.54 \\
GPT 2.0 (medium size): 40.31 \\

\textbf{Document level}: \\
GPT 2.0 (medium size): 36.84 \\
GPT 2.0 with context (medium size): 34.2 \\


\textbf{WikiText-2}: \\
it only has document level language model.
it doesn't have overlap with \cite{radford2019language} as demonstrated by GPT 2.0.

state of the art: 39.14\\
GPT 2.0 (medium size): 22.76 \\
GPT 2.0 with context (medium size): 21.03 \\


\textbf{WikiText-103}: \\
it only has document level language model.
it doesn't have overlap with \cite{radford2019language} as demonstrated by GPT 2.0.

state of the art: 18.3 \\
%GPT 2.0 (medium size): 26.37 \\
GPT 2.0 with context (medium size): 24.12 \\

}

\end{comment}





\begin{comment}

use Giga word as example, we can fine-tune the model.

small GPT 2.0 model \\

zero-shot: 12 layers with context: 33
zero-shot: 12 layers without context: 43 

even smaller model trained from scratch: \\

n\_embd = 384,n\_head = 6,n\_layer = 6,

0: train without context, test without context: 58
1: train without context, test with context: 52 
2: train with context, test without context: 67
3: train with context, test with context: 53$\leftrightarrow$39.9$\leftrightarrow$33.6 (epochs)

n\_embd = 384,n\_head = 6,n\_layer = 4,

0: train without context, test without context: 72
1: train without context, test with context: 69 
2: train with context, test without context: 78
3: train with context, test with context: 52

\end{comment}



\begin{comment}
NYT\_ENG\_20081222.0201.story, APW\_ENG\_20081223.0102.story: ok \\
NYT\_ENG\_20080314.0136.story, LTW\_ENG\_20080326.0068.story: ok \\
NYT\_ENG\_20080107.0001.story, APW\_ENG\_20080108.0270.story: ok \\
NYT\_ENG\_20080304.0205.story, APW\_ENG\_20080304.0735.story: bad \\
NYT\_ENG\_20080502.0157.story, APW\_ENG\_20080502.1121.story: ok \\
NYT\_ENG\_20080207.0237.story, LTW\_ENG\_20080209.0103.story: ok \\
NYT\_ENG\_20080418.0090.story, LTW\_ENG\_20080418.0110.story: ok \\ 
NYT\_ENG\_20081028.0159.story, APW\_ENG\_20081016.0217.story: ok \\ 
NYT\_ENG\_20080825.0167.story, APW\_ENG\_20080826.0929.story: ok \\
NYT\_ENG\_20080205.0130.story, XIN\_ENG\_20080205.0195.story: ok \\
\end{comment}
